Intelligent tutoring systems by Bayesian nets with noisy gates

Directed graphical models such as Bayesian nets are often used to implement intelligent tutoring systems able to interact in real-time with learners in a purely automatic way. When coping with such models, keeping a bound on the number of parameters might be important for multiple reasons. First, as these models are typically based on expert knowledge, a huge number of parameters to elicit might discourage practitioners from adopting them. Moreover, the number of model parameters affects the complexity of the inferences, while a fast computation of the queries is needed for real-time feedback. We advocate logical gates with uncertainty for a compact parametrization of the conditional probability tables in the underlying Bayesian net used by tutoring systems. We discuss the semantics of the model parameters to elicit and the assumptions required to apply such approach in this domain. We also derive a dedicated inference scheme to speed up computations.

==> 06_casestudy.tex <==
\section{A Case Study on K-12 Computational Skills}
We present here a case study where the noisy-AND structure models the \emph{Cross Array Task} (CAT) conceived by \cite{piatti_2022} to assess the algorithmic skills of compulsory school pupils. The tasks assigned to the pupils consists in providing the evaluator the necessary instructions to color an empty cross array in each of the twelve cross patterns in Fig. \ref{fig:its} (top). This task might be based on six binary skills meaning the pupil being able to use: simple patterns (e.g., columns, rows and squares) ($X_1$); complex patterns (e.g., diagonal and L-shape) ($X_2$); repetitions ($X_3$); symmetries ($X_4$); only the voice to communicate the algorithm ($X_5$); predict the outcome of the given instructions ($X_6$). Pupils can solve the task using different tools, namely their voice ($V$) to provide instructions, the combination of voice and an empty schema ($S$) to indicate the dots to be colored if skill 5 is weak, or, if also skill 6 is weak, the combination of voice, empty schema and a feedback ($F$) consisting in seeing how the evaluator is filling up the cross array. Moreover, the task can end in different algorithms classified as $A_2$ if they exploit repetitions and $A_1$ otherwise.

We consider tasks defined by the six (task, algorithm) combinations (and meaning  \textit{solving the CAT using a tool and ending in a algorithm of given type}). Questions from $Y_1$ to $Y_6$ are ordered based on their difficulty as follows: $(V,A_2)\!\succ \!(V,A_1)\!\succ\! (S,A_2)\!\succ\! (S,A_1)\!\succ\! (F,A_2)\!\succ\! (F,A_1)$. Assuming the solution given by a pupil described by task $Y_j$, we set $Y_j=1$ and assume all nodes corresponding to easier tasks (i.e., $Y_k$ with $k>j$) as not observed, and all tasks more difficult than $j$ as failed, i.e., $Y_k=0$ for all $k<j$.

Uniform PMFs are specified for the skills, whereas a domain expert elicited the strength $1-\lambda_{i,j}$ of the skill-question relations. Our succinct elicitation setup allows to summarize both the BN topology and quantification as in Fig. \ref{fig:its} (bottom). The questions associated with CATs 1 and 2 are the only non leaky models. A leaky model with $1-\lambda_0=0.2$ has been used for the questions associated with CATs 3 to 6, one with $1-\lambda_0=0.4$  for CATs 7 to 11 and one with $1-\lambda_0=0.7$ for CAT 12.

\begin{figure*}[ht]
\centering
\begin{tikzpicture}[]
\tikzset{b/.style={draw,circle,scale=0.3,blue!40!gray,fill}}
\tikzset{g/.style={draw,circle,scale=0.3,yellow,fill}}
\tikzset{r/.style={draw,circle,scale=0.3,red!80!gray,fill}}
\tikzset{v/.style={draw,circle,scale=0.3,green!40!gray,fill}}
\tikzset{l4/.style={draw,rectangle,scale=0.3,black!90,fill}}
\tikzset{l3/.style={draw,rectangle,scale=0.3,black!50,fill}}
\tikzset{l2/.style={draw,rectangle,scale=0.3,black!30,fill}}
\tikzset{l1/.style={draw,rectangle,scale=0.3,black!10,fill}}
\tikzset{l0/.style={draw,rectangle,scale=0.3,black!0,fill}}
\matrix[matrix of nodes,row sep=0.5mm,column sep=0.5mm]
{
&&&|[b]|&|[b]|&&&&
&&|[b]|&|[g]|&&&&
&&|[g]|&|[r]|&&&&
&&|[b]|&|[g]|&&&&
&&|[g]|&|[b]|&&&&
&&|[b]|&|[v]|&&&&
&&|[g]|&|[r]|&&&&
&&|[g]|&|[r]|&&&&
&&|[b]|&|[v]|&&&&
&&|[b]|&|[b]|&&&&
&&|[b]|&|[b]|&&&&
&&|[b]|&|[v]|\\
&&&|[b]|&|[b]|&&&&
&&|[b]|&|[g]|&&&&
&&|[g]|&|[r]|&&&&
&&|[b]|&|[g]|&&&&
&&|[g]|&|[b]|&&&&
&&|[b]|&|[v]|&&&&
&&|[r]|&|[g]|&&&&
&&|[r]|&|[b]|&&&&
&&|[r]|&|[g]|&&&&
&&|[g]|&|[g]|&&&&
&&|[v]|&|[v]|&&&&
&&|[r]|&|[g]|\\
&|[b]|&|[b]|&|[b]|&|[b]|&|[b]|&|[b]|&&
|[b]|&|[b]|&|[b]|&|[g]|&|[g]|&|[g]|&&
|[g]|&|[r]|&|[g]|&|[r]|&|[g]|&|[r]|&&
|[g]|&|[r]|&|[b]|&|[g]|&|[r]|&|[b]|&&
|[r]|&|[r]|&|[g]|&|[b]|&|[v]|&|[v]|&&
|[b]|&|[b]|&|[b]|&|[v]|&|[v]|&|[v]|&&
|[g]|&|[r]|&|[g]|&|[r]|&|[g]|&|[r]|&&  
|[g]|&|[r]|&|[g]|&|[r]|&|[g]|&|[r]|&&
|[b]|&|[v]|&|[b]|&|[v]|&|[b]|&|[v]|&&
|[g]|&|[b]|&|[g]|&|[g]|&|[b]|&|[g]|&&
|[v]|&|[b]|&|[r]|&|[r]|&|[b]|&|[v]|&&
|[g]|&|[v]|&|[b]|&|[v]|&|[b]|&|[r]|\\
&|[b]|&|[b]|&|[b]|&|[b]|&|[b]|&|[b]|&& 
|[b]|&|[b]|&|[b]|&|[g]|&|[g]|&|[g]|&&
|[g]|&|[r]|&|[g]|&|[r]|&|[g]|&|[r]|&&
|[g]|&|[r]|&|[b]|&|[g]|&|[r]|&|[b]|&&
|[r]|&|[r]|&|[g]|&|[b]|&|[v]|&|[v]|&&
|[g]|&|[g]|&|[g]|&|[r]|&|[r]|&|[r]|&&
|[r]|&|[g]|&|[r]|&|[g]|&|[r]|&|[g]|&& 
|[r]|&|[b]|&|[r]|&|[b]|&|[r]|&|[b]|&&
|[r]|&|[g]|&|[r]|&|[g]|&|[r]|&|[g]|&&
|[b]|&|[g]|&|[b]|&|[b]|&|[g]|&|[b]|&&
|[r]|&|[r]|&|[g]|&|[g]|&|[r]|&|[r]|&&
|[b]|&|[r]|&|[v]|&|[b]|&|[g]|&|[v]|\\
&&&|[b]|&|[b]|&&&&&&|[b]|&|[g]|&&&& 
&&|[g]|&|[r]|&&&&&&|[b]|&|[g]|&&&&
&&|[g]|&|[b]|&&&&&&|[g]|&|[r]|&&&&
&&|[g]|&|[r]|&&&&&&|[g]|&|[r]|&&&&
&&|[b]|&|[v]|&&&&&&|[b]|&|[b]|&&&&
&&|[b]|&|[b]|&&&&&&|[g]|&|[r]|\\
&&&|[b]|&|[b]|&&&&&&|[b]|&|[g]|&&&& % Schema 1 2
&&|[g]|&|[r]|&&&&&&|[b]|&|[g]|&&&&
&&|[g]|&|[b]|&&&&&&|[g]|&|[r]|&&&&
&&|[r]|&|[g]|&&&&&&|[r]|&|[b]|&&&& % Schema 7 8 
&&|[r]|&|[g]|&&&&&&|[g]|&|[g]|&&&&
&&|[g]|&|[g]|&&&&&&|[r]|&|[g]|\\
&&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}&
&&&&&&\phantom{\tiny{...}}\\
&|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&	
|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&	
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&	
|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&	
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&	
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&	
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&	
|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&	
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|\\
&|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&	
|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&	
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&	
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&	
|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&	|[l1]|&	|[l2]|&&	
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&	
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&	
|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&	|[l3]|&	|[l4]|&&	
|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&&	
|[l3]|&	|[l1]|&	|[l3]|&	|[l1]|&	|[l3]|&	|[l1]|&&	
|[l2]|&	|[l3]|&	|[l2]|&	|[l3]|&	|[l2]|&	|[l3]|&&	
|[l0]|&	|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l3]|\\
&|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&	
|[l2]|&	|[l0]|&	|[l2]|&	|[l0]|&	|[l2]|&	|[l0]|&&	
|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&&	
|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&&	
|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&	
|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&	
|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&&	
|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&&	
|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&	|[l4]|&	|[l0]|&&	
|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&&
|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&&	
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|\\
&|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&
|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&
|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&
|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&
|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&	|[l1]|&	|[l0]|&&
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&&
|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&&
|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l3]|&	|[l0]|&&
|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|&	|[l0]|\\
&|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&	|[l0]|&	|[l0]|&&	
|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&	|[l0]|&	|[l0]|&&	
|[l3]|&	|[l3]|&	|[l1]|&	|[l1]|&	|[l0]|&	|[l0]|&&	
|[l3]|&	|[l3]|&	|[l1]|&	|[l1]|&	|[l0]|&	|[l0]|&&	
|[l3]|&	|[l3]|&	|[l1]|&	|[l1]|&	|[l0]|&	|[l0]|&&	
|[l4]|&	|[l4]|&	|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&&	
|[l4]|&	|[l4]|&	|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&&	
|[l4]|&	|[l4]|&	|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&&	
|[l4]|&	|[l0]|&	|[l2]|&	|[l0]|&	|[l1]|&	|[l0]|&&	
|[l4]|&	|[l4]|&	|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&&	
|[l4]|&	|[l4]|&	|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&&	
|[l0]|&	|[l4]|&	|[l0]|&	|[l2]|&	|[l0]|&	|[l1]|\\
&|[l2]|&	|[l2]|&	|[l1]|&	|[l1]|&	|[l0]|&	|[l0]|&&
|[l2]|&	|[l2]|&	|[l2]|&	|[l2]|&	|[l0]|&	|[l0]|&&
|[l3]|&	|[l3]|&	|[l2]|&	|[l2]|&	|[l0]|&	|[l0]|&&
|[l3]|&	|[l3]|&	|[l2]|&	|[l2]|&	|[l0]|&	|[l0]|&&
|[l3]|&	|[l3]|&	|[l2]|&	|[l2]|&	|[l0]|&	|[l0]|&&
|[l3]|&	|[l3]|&	|[l2]|&	|[l2]|&	|[l0]|&	|[l0]|&&
|[l4]|&	|[l4]|&	|[l3]|&	|[l3]|&	|[l0]|&	|[l0]|&&
|[l4]|&	|[l4]|&	|[l3]|&	|[l3]|&	|[l0]|&	|[l0]|&&
|[l4]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l0]|&	|[l0]|&&
|[l4]|&	|[l4]|&	|[l3]|&	|[l3]|&	|[l0]|&	|[l0]|&&
|[l4]|&	|[l4]|&	|[l3]|&	|[l3]|&	|[l0]|&	|[l0]|&&
|[l0]|&	|[l4]|&	|[l0]|&	|[l3]|&	|[l0]|&	|[l0]|\\
};
\end{tikzpicture}
\caption{The twelve cross array schemes (top) and elicitation of the corresponding tasks (bottom). For each schema, the elicitation is depicted as a matrix of squares with six rows (one for each skill) and six columns (one for each question). The strength of the skill-question relation has four levels, namely, $1-\lambda_{i,j} \in \{0.2, 0.4, 0.7, 0.9\}$, with darker shades of gray meaning higher strengths. White squares denote non-relevant skills (i.e., $1-\lambda_{i,j}=0$) corresponding to missing skill-to-question arcs.}\label{fig:its}
\end{figure*}

The underlying BN has been implemented within the CREMA Java library \cite{huber2020a}. CREMA supports the specification of noisy gates and inference based on these parametric CPTs.

We processed the answers of 15 pupils and four of them are discussed here as representative examples (Tab. \ref{tab:results}). The first three pupils solved the tasks only by voice, whereas the fourth required all the helps for CATs 11 and 12 and solved by voice alone only the trivial CAT 1. Therefore, the first three students are assigned a very high probability for voice ($X_5$) and prediction ($X_6$), whereas for the fourth pupil they are almost zero. The first pupil failed CATs 8 to 12, the second CATs 7,8,9 and 12, the third CAT 12 and the fourth CATs 6,8,9,10. Therefore, only the third pupil was able to solve almost all schemes with complex patterns (namely, 8 to 12) and was therefore given a high posterior for \emph{complex patterns} ($X_2$). All pupils got a high probability for \emph{simple patterns} ($X_1$) except for the third, as she/he needed help even in the easiest schemes. Concerning \emph{repetitions} ($X_3$), since only the third pupil solved with repetitions CATs 7 to 9 (for which repetitions are essential), for her/him alone that skill received a high probability. Of the other three pupils, assigned with a posterior for $X_3$ close to zero, the first used a $A_2$ algorithm only in the relatively simple CAT 7, the second only in CATs 10 and 11 (i.e., those where symmetries are more relevant than repetitions in the $A_2$ algorithm), and the fourth always ended in a $A_1$ algorithms. Finally, \textit{symmetries} ($X_4$) is large only for the second pupil, being the only one able to solve CATs 10 and 11 in $A_2$.

These results show how it is possible to effectively apply noisy gates to non trivial assessment tasks, enabling the automatic assessment of the learner during a learning process. 
\begin{table}[htb]
\centering
\begin{tabular}{ccccccc}
\toprule
& \multicolumn{6}{c}{\textbf{$P(X_i=1|\bm{y}^{(j)})$}}\\ 
$j$&{\footnotesize $i=1$}&{\footnotesize $i=2$}&{\footnotesize $i=3$}&{\footnotesize $i=4$}&{\footnotesize $i=5$}&{\footnotesize $i=6$}\\
\midrule
1 & 0.93 & 0.02 & 0.06 & 0.19 & 0.94 & 0.85 \\
2 & 1.00 & 0.00 & 0.08 & 0.90 & 1.00 & 0.99 \\
3 & 1.00 & 1.00 & 1.00 & 0.39 & 1.00 & 1.00 \\
4 & 0.45 & 0.00 & 0.00 & 0.15 & 0.00 & 0.01 \\
\bottomrule
\end{tabular}
\caption{Pupil skill posterior probabilities. The answers provided by the $j$-th pupil are denoted as $\bm{y}^{(j)}$.\label{tab:results}}
\end{table}
